Improving frequency response with synthetic damping available from fleets of distributed energy resources

With the increasing use of renewable generation in power systems, responsive resources will be necessary to support primary frequency control in future low-inertia/under-damped power systems. Flexible loads can provide fast-frequency response services if coordinated effectively. However, practical implementations of such synthetic damping services require both effective local sensing and control at the device level and an ability to accurately estimate online and predict the available synthetic damping from a fleet. In addition, the inherent trade-off between a fleet being available for fast frequency response while providing other ancillary services needs to be characterized. In this context, the manuscript presents a novel, fully decentralized, packet-based controller for diverse flexible loads that dynamically prioritizes and interrupts loads to engender synthetic damping suitable for primary frequency control. Moreover, the packet-based control methodology is shown to accurately characterize the available synthetic damping in real-time, which is useful to aggregators and system operators. Furthermore, spectral analysis of historical frequency regulation data is used to produce a probabilistic bound on the expected available synthetic damping for primary frequency control from a fleet and the trade-off from concurrently providing secondary frequency control services. Finally, numerical simulation on IEEE test networks demonstrates the effectiveness of the proposed methodology.

==> Old_files/CSSPreamble.tex <==
%%% ============================================================================================================= %%%
%%%                                  The lastest updated date: November 11th, 2004                                    %%%
%%% ============================================================================================================= %%%
%%% Update Log: 11/16/2004, add the \RomanNumber and \romannumber for capital and small Roman numbers
%%%                         add \rb for table raising box
%%% Update Log: 05/08/2004, add the matlab and simulink definition in the end for reference
%%% Update Log: 04/26/2004, add the math operator ``dist'', update the definition for theorem-like enviroments
%%% Update Log: 03/04/2004, use package 'upgreek' for constants, e.g., $\uppi$ = 3.1415926.... (ISO standard)
%%% Update Log: 09/12/2004, update for solving the conflicts between amsthm and cssconf
%%% ============================================================================================================= %%%

\usepackage{latexsym, amssymb, amsmath}
%\usepackage[dvips]{graphicx} % added for inserting the pictures
%% \usepackage[dvips]{color}
%% \usepackage{amsthm}
%% \usepackage{amscd}% amscd for "commutative diagram"
\usepackage{enumerate}
%% \usepackage{url}
%\usepackage{upref} % make all ref's are upright fonttype, no use in this paper % zzz: removed by Dr. Gray and Dr. Gonzalez
%% \usepackage{upgreek} % use upright greek to represent constant values, i.e., $\uppi$ = 3.14, ...
%\usepackage{flushend} % align at the last lines of every page
\usepackage{mathrsfs} % added by Hong for Script Capital Letters by using "$\mathscr{}$"
%% \usepackage{easybmat} % A simple package for writing block matrices with equal column widths or equal rows heights or both, with various kinds of rules between rows and columns.
%% \usepackage{txfonts}%, pxfonts
%% \usepackage{euscript} %, amsfonts}
%% \usepackage{times}
%% \usepackage{color}
%\usepackage{stfloats}
%% \usepackage{float}
%% Packages added by Dr. Gonzalez
%\usepackage{indentfirst}    %Automatically indents the beginning of the paragraph following a Latex section
\usepackage{cite}
%%% ============================================================================================================= %%%

% Hong's setting for figures for this paper
%\setlength{\textfloatsep}{.3em}
%\setlength{\intextsep}{.5em}

% Reduce Space Between Paragraphs
%\setlength{\parskip}{1.5ex} %plus 1pt minus 1pt}

% Reduce Space Above and Below Equations
%\setlength{\jot}{-0.7pt} % eqnarray extra space
%\setlength{\abovedisplayskip}{-1pt}% plus 1pt minus 1pt} % extra space above eqn
%\setlength{\abovedisplayshortskip}{-1pt}% plus 1pt minus 1pt} % extra space above eqn
%\setlength{\belowdisplayskip}{-1pt}% plus 1pt minus 1pt} % extra space below eqn
%\setlength{\belowdisplayshortskip}{-1pt}% plus 1pt minus 1pt} % extra space below eqn
%\setlength{\topsep}{0.2pt}

% Insert Breaks Between a Long Formula
%\allowdisplaybreaks[3] % added by Hong for allowing page breaks among a large formula


%%% ============================================================================================================= %%%
% new theorems environment
%\swapnumbers
%% \theoremstyle{plain} % default
\newtheorem{prop}{Proposition} % [section]
\newtheorem{proposition}[prop]{Proposition} % [section]
\newtheorem{lem}{Lemma} % [section]
\newtheorem{lemma}[lem]{Lemma} % [section]
\newtheorem{thm}{Theorem} % [section]
\newtheorem{theorem}[thm]{Theorem} % [section]
\newtheorem{cor}{Corollary} % [section]
\newtheorem{corollary}[cor]{Corollary} % [section]
%\newtheorem{exer}{Exercise}[section]
%\newtheorem{test}{Test}[section]

%% \theoremstyle{definition}
\newtheorem{defn}{Definition} % [section]
\newtheorem{defi}[defn]{Definition} % [section]
\newtheorem{definition}[defn]{Definition} % [section]
\newtheorem{conj}{Conjecture} % [section]
\newtheorem{exmp}{Example} % [section]
\newtheorem{example}[exmp]{Example} % [section]
\newtheorem{exam}[exmp]{Example} % [section]
\newtheorem{exam*}{Example}

%% \theoremstyle{remark}
%% \newtheorem*{rmk}{Remark}
%% \newtheorem*{remark}{Remark}
% %\newtheorem*{note}{Note}
% \newtheorem{case}{Case}

% \newtheoremstyle{model}% name
%   {3pt}%      Space above, empty = `usual value'
%   {3pt}%      Space below
%   {\itshape}% Body font
%   {}%         Indent amount (empty = no indent, \parindent = para indent)
%   {\textnormal}% Thm head font
%   {.}%        Punctuation after thm head
%   {.5em}%     Space after thm head: " " = normal interword space;
%         %       \newline = linebreak
%   {}% Thm head spec
%\renewcommand {\thmhead}[3]{\thmname{#1}\thmnumber{#2}\thmnote{\textnormal{[\emph{#3}]}}}

% \theoremstyle{model}
% \newtheorem*{mdl}{Rollback Interference Model}


%%% ============================================================================================================= %%%
%% Generates a bibliography with 'References' centered above the column, changed by Hong
%\def\custombibliography#1{
% \normalsize
%% The part was commented by Hong
%% \begin{center}
%% {\Large \bf{References}}
%% \end{center}
%\section*{\centering References}
% \list
% {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
% \setlength{\itemsep}{.1em}
% \advance\leftmargin\labelsep
% \usecounter{enumi}}
% \def\newblock{\hskip .11em plus .33em minus -.07em}
% \sloppy
% \sfcode`\.=1000\relax}
%\let\endthebibliography=\endlist


%%% ============================================================================================================= %%%
% Gray's Abbreviations
\def\L2{{\cal L}_2}
\def\begar{\begin{array}}
\def\endar{\end{array}}
\def\begce{\begin{center}}
\def\endce{\end{center}}
\def\begco{\begin{cor}}
\def\endco{\end{cor}}
\def\begde{\begin{defn}}
\def\endde{\end{defn}}
\def\begdes{\begin{description}}
\def\enddes{\end{description}}
\def\begdi{\begin{displaymath}}
\def\enddi{\end{displaymath}}
\def\begdis{\begin{eqnarray*}}
\def\enddis{\end{eqnarray*}}
\def\begen{\begin{enumerate}}
\def\enden{\end{enumerate}}
\def\begeq{\begin{equation}}
\def\endeq{\end{equation}}
\def\begeqa{\begin{eqnarray}}
\def\endeqa{\end{eqnarray}}
\def\begex{\begin{exmp}}
\def\endex{\end{exmp}}
\def\begfig{\begin{fig}}
\def\endfig{\end{fig}}
\def\begit{\begin{itemize}}
\def\endit{\end{itemize}}
\def\begle{\begin{lem}}
\def\endle{\end{lem}}
\def\begpro{\begin{prop}} % added by Hong
\def\endpro{\end{prop}} % added by Hong
\def\begth{\begin{thm}}
\def\endth{\end{thm}}
\def\begre{\noindent{\em Remark}:\ } % changed by Hong
\def\endre{\\}
\def\begres{\noindent{\em Remarks}:\begin{enumerate}}
\def\endres{\end{enumerate} \par}
\def\begpr{\begin{proof}} % changed by Hong
\def\endpr{\end{proof}}
%\def\begpr{\noindent{\em Proof}\ : } % changed by Hong
%\def\endpr{\hspace*{0.05in}\bull\vspace*{0.15in}\\}
%\def\beglar{\left[\begin{array}}
%\def\endrar{\end{array}\right]}


%%% ============================================================================================================= %%%
% Gray's New Commands
\newcommand\bull{\vrule height .9ex width .8ex depth -.1ex } % square bullet
\newcommand\bul{$\bullet\;\;\;$}
\newcommand\re{\rm I\! R}
%\renewcommand\qed{\hfill$\Box \Box \Box$}
%\newcommand\mathbfsub#1{\hbox{\mathversion{bold}$\scriptstyle #1$}} % Stopped by Hong; Define better command \rv
%\newcommand\rref[1]{(\ref{#1})} % Stopped by Hong; Use AMS LaTeX command \eqref
\newcommand\spacebox[1]{\raisebox{-6pt}[7pt][0pt]{#1}} % puts extra space around items in a table
\newcommand\cdcout[1]{} % reduce it to 6 pages
%\newcommand\cdcout[1]{#1} % restores the CDC 7 page version


%%% ============================================================================================================= %%%
% Hong's Abbreviations for Left and Right Delimiters
\newcommand{\Lb}{\left [}          % Left bracket
\newcommand{\Rb}{\right ]}         % Right bracket
\newcommand{\LB}{\left \{}         % Left brace
\newcommand{\RB}{\right \}}        % Right brace
\newcommand{\Ld}{\left .}          % Left default
\newcommand{\Rd}{\right .}         % Right default
\newcommand{\Lp}{\left (}          % Left parenthese
\newcommand{\Rp}{\right )}         % Right parenthese
\newcommand{\Lv}{\left |}          % Left vertical line
\newcommand{\Rv}{\right |}         % Right vertical line
\newcommand{\LV}{\left \|}         % Left vertical double line
\newcommand{\RV}{\right \|}        % Right vertical double line


%%% ============================================================================================================= %%%
% Hong's New Commands and Declarations for Linear Algebra and Matrix Analysis
\DeclareMathOperator{\trace}{tr}   % Define a matrix' trace operator, sometimes
\DeclareMathOperator{\diag}{diag}  % Define the diagonal matrix operator
\DeclareMathOperator{\rank}{rank}  % Define the rank operator of a matrix
\DeclareMathOperator{\vect}{vec}   % Define the function to reshape a matrix into a vector column-wise.
% \DeclareMathOperator{\col}{col}    % Define the column operator, e.g., $cy = \col \LB y_i, \dots, y_n \RB$
\newcommand{\T}{^\mathrm{T}}       % Transposition operator of the matrix or vector
\newcommand{\h}{^\mathrm{H}}       % Hermitian Transposition of a matrix or vector


%%% ============================================================================================================= %%%
% Hong's New Commands and Declarations for Random Variables, Probability and Stochastic Process
\newcommand{\rv}[1]{\boldsymbol{#1}} % Use italic boldface to indicate the Random Variables
\DeclareMathOperator{\Var}{Var}      % Operator for variance of a RV
\DeclareMathOperator{\Cov}{Cov}      % Operator for covariance of a RV
\DeclareMathOperator*{\Lim}{l.i.m.}  % Operator for convergence in the MS sense

%%% ============================================================================================================= %%%
% Hong's New Commands and Declarations for Mathematical Analysis and Other Areas
\DeclareMathOperator{\sgn}{sgn}      % Operator for sign function
\DeclareMathOperator*{\argmax}{\arg\max}
\DeclareMathOperator{\dist}{dist}

%%% ============================================================================================================= %%%
%% New Commands for Sets or Spaces
\newcommand{\N}{\mathbb N} % for the set of natural
\newcommand{\C}{\mathbb C} % for the set of complex
\newcommand{\Q}{\mathbb Q} % for the set of rational
\newcommand{\R}{\mathbb R} % for the set of real
\newcommand{\Z}{\mathbb Z} % for the set of integer

%%% ============================================================================================================= %%%
% International Typesetting Standards
\newcommand{\me}{\mathrm{e}} % for math e
\newcommand{\mi}{\mathrm{i}} % for math i
\newcommand{\mj}{\mathrm{j}} % added by Hong for engineering j
\newcommand{\dif}{\,\mathrm{d}}% for differential

%%% ============================================================================================================= %%%
%% Hong's abbreviations of sets or spaces for this paper
\newcommand{\MRn}{\mathbb M(\R^{n})}
\newcommand{\Hn}{\mathbb H^n}
\newcommand{\Hnp}{\mathbb H^{n+}}
\newcommand{\BHn}{\mathbb B(\Hn)}

%%% ============================================================================================================= %%%
%% Hong's other settings just for this paper
%% \renewcommand{\labelenumi}{\textup{(\alph{enumi})}}
%% \setlength{\topsep}{-1pt}
%%\setlength{\itemsep}{-5pt}

%%% ============================================================================================================= %%%
%% Hong's other commands
\newcommand{\matlab}{\textsc{MATLAB}\textsuperscript{\textregistered}} % for the mathworks MATLAB registered product
\newcommand{\simulink}{Simulink\textsuperscript{\textregistered}} % for the mathworks Simulink registered product

%%% ============================================================================================================= %%%
%% Hong's Capital/Small Roman Numbers
\newcommand{\RomanNumber}[1]{\uppercase\expandafter{\romannumeral #1}}
\newcommand{\romannumber}[1]{\lowercase\expandafter{\romannumeral #1}}

%%% ============================================================================================================= %%%
%% Hong's Fonts definitions

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

%% Table Raising box
\newcommand{\rb}[1]{\raisebox{1.5ex}[0pt]{#1}}

%%% ============================================================================================================= %%%
%% Dr. Gonzalez's Group definitions
\def\1{\rv 1} %Indicator
\def\I{{\mathcal I}}    %Index set
\def\E{{\mathbb E}}    %PDP state space
\def\bE{{\mathcal E}}    %Borel set
\def\x{{\rv\chi}}    %hybrid PDP state
\def\B{{\mathcal B}}    %Index set


%\renewcommand{\baselinestretch}{0.94}

==> Old_files/abbreviations.tex <==

% Master List of Latex Abbreviations

% Color Abbreviations
%
\def\bluetext#1{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
\def\blacktext#1{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\def\redtext#1{\textcolor[rgb]{0.98,0.00,0.00}{#1}}
\def\yellowtext#1{\textcolor[rgb]{1.00,1.00,0.26}{#1}}
\def\whitetext#1{\textcolor[rgb]{1.00,1.00,1.0}{#1}}
\def\colornote#1{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\definecolor{Light}{gray}{0.85}

% Symbol Abbreviations

% Aa
\def\adj{{\rm adj}}
\def\abs#1{\left\vert #1 \right\vert}
%
\def\allcommutingpoly{\mbox{$\re[X]$}}
% Want to make these obsolete to avoid conflict in second group, item 3
\def\allcommutingseries{\mbox{$\re\, [[\tilde{X}]]$}}
\def\allcommutingseriesell{\mbox{$\re^{\ell}\, [[\tilde{X}]]$}}
\def\allcommutingseriesellLC{\mbox{$\re^{\ell}_{LC}\, [[\tilde{X}]]$}}
\def\allcommutingseriesm{\mbox{$\re^{m}\, [[\tilde{X}]]$}}
%-----------------------------------------------------------------------
\def\allcommutingseriestildem{\mbox{$\re^{\tilde{m}}\, [[X]]$}}
\def\allcommutingseriestildeXell{\mbox{$\re^{\ell}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXtildeell{\mbox{$\re^{\tilde{\ell}}\, [[\tilde{X}]]$}}
\def\allcommutingseriesX{\mbox{$\re\, [[X]]$}} % X is nonstandard
\def\allcommutingseriesXell{\mbox{$\re^{\ell}\, [[X]]$}} % X is nonstandard
\def\allcommutingseriesXOell{\mbox{$\re^{\ell}\, [[X_0]]$}}
\def\allcommutingseriesXO{\mbox{$\re_{LC}\, [[X_0]]$}}
%
\def\allpoly{\mbox{$\re\langle X \rangle$}}
\def\allpolyell{\mbox{$\re^{\ell}\langle X \rangle$}}
%\def\allpolyx0{\mbox{$\re[[ x_0 ]]$}} % This convention is obsolete
\def\allpolyx0degn{\mbox{$P_n$}}
\def\allpolyXO{\mbox{$\re [X_0]$}}
\def\allpolyXOm{\mbox{$\re^m [X_0]$}}
\def\allpolyXW{\mbox{$\re\langle XW \rangle$}}
%\def\allpolyI{\mbox{$\re\langle I \rangle$}} % This convention is obsolete
%
\def\allseries{\mbox{$\re\langle\langle X \rangle\rangle$}}
\def\allseriesdelta{\mbox{$\re\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesell{\mbox{$\re^{\ell} \langle\langle X \rangle\rangle$}}
\def\allseriesGC{\mbox{$\re_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriesLC{\mbox{$\re_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesm{\mbox{$\re^m\langle\langle X \rangle\rangle$}}
\def\allseriesmtimesm{\mbox{$\re^{m\times m}\langle\langle X \rangle\rangle$}}
\def\allseriesmDF{\mbox{$\re^m\langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriesmGC{\mbox{$\re^{m}_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriesmLC{\mbox{$\re^{m}_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesmLCDF{\mbox{$\re^{m}_{LC}\langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriesnLC{\mbox{$\re^{n}_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesn{\mbox{$\re^n\langle\langle X \rangle\rangle$}}
\def\allseriesntimesn{\mbox{$\re^{n\times n}\langle\langle X \rangle\rangle$}}
\def\allseriesSLC{\mbox{$\re_{LC}\langle\langle S \rangle\rangle$}}
\def\allZseries{\mbox{$\mathbb{Z}\langle\langle X \rangle\rangle$}}
%
\def\allseriestildeXtildeell{\mbox{$\re^{\tilde{\ell}} \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeell{\mbox{$\re^{\tilde{\ell}} \langle\langle X \rangle\rangle$}}
\def\allseriestildem{\mbox{$\re^{\tilde{m}} \langle\langle X \rangle\rangle$}}
\def\allseriestildeX{\mbox{$\re \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXell{\mbox{$\re^\ell \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXLC{\mbox{$\re^\ell_{LC} \langle\langle \tilde{X} \rangle\rangle$}}
%
\def\allseriesellLC{\mbox{$\re^{\ell}_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesellGC{\mbox{$\re^{\ell}_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriestwo{\mbox{$\re^{2}\langle\langle X \rangle\rangle$}}
\def\allseriestwoLC{\mbox{$\re^{2}_{LC}\langle\langle X \rangle\rangle$}}
% These are obsolete
%\def\allseriesI{\mbox{$\re\langle\langle I \rangle\rangle$}}
%\def\allseriesILC{\mbox{$\re_{LC}\langle\langle I \rangle\rangle$}}
%\def\allseriesIm{\mbox{$\re^m\langle\langle I \rangle\rangle$}}
%\def\allseriesImLC{\mbox{$\re^m_{LC}\langle\langle I \rangle\rangle$}}
%\def\allseriesIell{\mbox{$\re^{\ell}\langle\langle I \rangle\rangle$}}
%\def\allseriesIellLC{\mbox{$\re^{\ell}_{LC}\langle\langle I \rangle\rangle$}}
\def\allseriesx{\mbox{$\re[[x]]$}}
\def\allseriesXO{\mbox{$\re [[ X_0 ]]$}}
\def\allseriesXOLC{\mbox{$\re_{LC} [[ X_0 ]]$}}
\def\allseriesXOm{\mbox{$\re^m [[ X_0 ]]$}} % use oh since zero is not allowed
\def\allseriesXOmLC{\mbox{$\re^m_{LC} [[ X_0 ]]$}}
\def\allseriesXOell{\mbox{$\re^{\ell} [[ X_0 ]]$}}
\def\allseriesXOellLC{\mbox{$\re^{\ell}_{LC} [[ X_0 ]]$}}
\def\allseriesXWell{\mbox{$\re^{\ell}\!\ll\!XW\!\gg$}}
\def\allseriesXW{\mbox{$\re\!\ll\!XW\!\gg$}}
\def\allseriesXWLC{\mbox{$\re_{LC}\!\ll\!XW\!\gg$}}
\def\allseriesWLC{\mbox{$\re_{LC}\!\ll\!W\!\gg$}}
\def\allseriesXWellLC{\mbox{$\re^{\ell}_{LC}\!\ll\!XW\!\gg$}}
\def\allseriesX1{\mbox{$\re [[ X_1 ]]$}}
%
\def\alltransductionsXtildeX{\mbox{$[\allseriestildeX] \langle\langle X \rangle\rangle$}}

% Bb
\def\bfem#1{{\bf \em #1}} % boldface italics
\def\borel{\mathscr{B}}
\def\borelf{\mathscr{B}_f}
\def\Bp{B_{\mathfrak{p}}}
\def\Bpm{B_{\mathfrak{p}}^m}
\def\Bq{B_{\mathfrak{q}}}
\def\Bqell{B_{\mathfrak{q}}^\ell}
\def\Bqm{B_{\mathfrak{q}}^m}
\def\bull{\rule{0.08in}{0.08in}} % square filled bullet

% Cc
\def\C{{\mathbb C}} % complex numbers (AMS symbol)
\def\Cc{{\cal C}} % class of continuous functions
\def\card{{\rm card}}
\def\charseries{{\rm char}}
\def\Chengroup{{\cal G}_C(\tilde{X})}
\def\Chenseries{{\cal G}_C(X)}
\def\chiup{\hbox{\raisebox{0.03in}{$\chi$}}} % slightly raised \chi symbol
\def\chiupsub{\hbox{\raisebox{0.02in}{$\scriptstyle \chi$}}} % slightly raised \chi symbol
\newcommand{\comment}[1]{} % allows one to comment out a block of text
\def\conc{{\rm cat}}

% Dd
\def\diag{{\rm diag}}
\def\dim{{\rm dim}}
\def\dist{{\rm dist}}
\def\down#1{{}_{{}_{#1}}}
\def\doubleone{{\rm\, l\!l}}

% Ee
\def\EndoA{{\rm End}($A$)}
\def\Endallseries{{\rm End}(\allseries)}
\def\eqref#1{(\ref{#1})} % parentheses around referenced equation numbers
%\def\equivf{\underset{f}{\sim}} % Does not match Chapter 1 format
\def\equivf{{\sim_f}}
\DeclareMathOperator*{\esssup}{ess\;\, sup}
\def\expdown{{\rm exp}}
\def\expup{{\rm e}}

% Ff
\def\fac{{\rm fac}}
\def\Fliessdelta{\mathscr{F}_{\delta}}
\def\FliessLC{\mathscr{F}}
\def\freegroup{{\cal F}}

% Gg
\def\GLn{GL_n(\re)}
\def\groupE{{\cal G}(E)}

% Hh
\newcommand{\hX}{\hat X}
\newcommand{\hW}{\hat W}

% Ii
\def\integers{{\mathbb Z}} % integers
\def\im{{\rm im}}
\def\impart{{\rm Im}}
\def\innprod#1#2{\left\langle #1, #2 \right\rangle}

% Kk
\def\ker{{\rm ker}}

% Ll
\def\Lp{L_{\mathfrak{p}}}
\def\Lpm{L_{\mathfrak{p}}^m}
\def\Lpe{L_{\mathfrak{p},e}}
\def\Lpme{L^m_{\mathfrak{p},e}}
\def\Lq{L_{\mathfrak{q}}}
\def\Lqell{L_{\mathfrak{q}}^\ell}
\def\Lqm{L_{\mathfrak{q}}^m}
\def\laplace{\mathscr{L}}
\def\laplacef{\mathscr{L}_f}
\def\liead{{\rm ad}}
\def\tliead{{\rm \widetilde{ad}}}
\def\lieAd{{\rm Ad}}
\def\tlieAd{{\rm \widetilde{Ad}}}
\def\liepoly{{\cal L}(X)}
\def\liepolyO{{\cal L}_0(X)}
\def\lieseries{\widehat{\cal L}(X)}

% Mm
\def\Magnusgroup{{\cal G}_M(X)}
\def\Malcevgroup{\widehat{\cal G}(X)}
\def\MalcevgrouptildeX{\widehat{\cal G}(\tilde{X})}
\def\mbf#1{\hbox{\mathversion{bold}$#1$}} % math boldface
\def\modcomp{\:\tilde{\circ}\,} % modified composition product

% Nn
\def\nat{{\mathbb N}} % natural numbers (AMS symbol)
\def\norm#1{\Vert#1\Vert}
\def\notin{{\not\in}}
\def\ns#1{{\textstyle #1}} % normalsize fonts in subscripts
\def\Null{{\rm null}}

% Oo
\def\openbull{\framebox[0.08in][c]{$\;$}} % square unfilled bullet
\def\ord{{\rm ord}}

% Pp
\def\preMalcevgroup{{\cal G}(X)}

% Qq
\def\qed{\hfill$\Box \Box \Box$}

% Rr
%\newcommand{\R}{\mathbb R}
\def\rank{{\rm rank}}
\def\rat{\re(s)}
\def\ratp{\re_p(s)}
\def\ratpone{\re_{p1}(s)}
\def\ratpnotO{\re_{p\bar{0}}(s)}
\def\ratsp{\re_{p0}(s)}
\def\re{{\mathbb R}} % real numbers (AMS symbol)
\def\repart{{\rm Re}}

% Ss
\def\sameau{\rule[0.017in]{0.2in}{0.012in}}
\def\sh{{\rm sh}}
%\def\shuffle{{\hbox{\cyr x}}} % shuffle product using cyrillic font
\def\shuffle{{\scriptscriptstyle \;\sqcup \hspace*{-0.05cm}\sqcup\;}}
\def\shuffleXW{{{\shuffle}}}
\font\grs=eurm10 at 9pt \def\smu{{\hbox{\grs\char22}}} % use for micro...
\def\spacebox#1{\raisebox{-3pt}[5pt][7pt]{#1}} % puts extra space around items in a table
\def\spanset{{\rm span}}
\def\supp{{\rm supp}}
\def\ss#1{{\scriptstyle #1}} % fonts in subsubscripts
\def\sss#1{{\scriptscriptstyle #1}} % fonts in subsubsubscripts

% Tt
\def\Tr{{\rm Tr}}

% Uu
\font\grg=eurm10 \def\umu{{\hbox{\grg\char22}}} % upright mu.

% Vv
\def\ve{\varepsilon}
\def\vec{{\rm vec}}

% Zz
\def\Ztransform{\mathscr Z}

% Environment Abbreviations
%
\def\begals{\[\begin{aligned}}
\def\endals{\end{aligned}\]}
\def\begce{\begin{center}}
\def\endce{\end{center}}
\def\begar{\begin{array}}
\def\endar{\end{array}}
\def\begeq{\begin{equation}}
\def\endeq{\end{equation}}
\def\begdi{\begin{displaymath}}
\def\enddi{\end{displaymath}}
\def\begdis{\begin{eqnarray*}}
\def\enddis{\end{eqnarray*}}
\def\begeqa{\begin{eqnarray}}
\def\endeqa{\end{eqnarray}}
\def\begdes{\begin{description}}
\def\enddes{\end{description}}
\def\begit{\begin{itemize}}
\def\endit{\end{itemize}}
\def\begen{\begin{enumerate}}
\def\enden{\end{enumerate}}
\def\beglar{\left[\begin{array}}
\def\endrar{\end{array}\right]}
\def\begle{\begin{mylemma}}
\def\endle{\end{mylemma}}
\def\begde{\begin{mydefinition}}
\def\endde{\end{mydefinition}}
\def\begth{\begin{mytheorem}}
\def\endth{\end{mytheorem}}
\def\begco{\begin{mycorollary}}
\def\endco{\end{mycorollary}}
\def\begprop{\begin{myproposition}}
\def\endprop{\end{myproposition}}
\def\begex{\begin{myexample}}
\def\endex{\hfill\openbull \end{myexample} \vspace*{0.15in}}
\def\begexer{\begin{myexercise}}
\def\endexer{\end{myexercise}}
\def\begre{\noindent{\em Remark}:}
\def\endre{\\}
\def\begres{\noindent{\em Remarks}:\begin{enumerate}}
\def\endres{\end{enumerate} \par}
\def\begpr{\noindent{\em Proof:}$\;\;$}
\def\endpr{\hfill\bull \vspace*{0.15in}}
\def\begtab{\begin{tabular}}
\def\endtab{\end{tabular}}
\def\rref#1{(\ref{#1})}
\def\problem#1{\vspace*{0.1in}\noindent {\bf Problem \ref{#1}}} % for the solution key
%\setlength{\marginparwidth}{1.25in} % controls width of margin notes
%\setlength{\marginparsep}{0.25in} % controls space between book text and margin note
%\def\marginnote#1{\marginpar{{\scriptsize\colornote{#1}}}} % margin note in red
%%\def\marginnote#1{\marginpar{{\scriptsize\whitetext{#1}}}} % margin note in white
%\def\pmarginnote#1{\marginpar{{\scriptsize\colornote{#1}}}} % private margin note, i.e., not shown in general

% Luis' Abbreviations for CDC 2007 insert
\def\allseriesY{\mbox{$\re\!\ll\!Y\!\gg$}}
\def\allseriesZ{\mbox{$\re\!\ll\!Z\!\gg$}}
\def\allseriestZj{\mbox{$\re\!\ll\!\tilde{Z}_j\!\gg$}}
\def\allseriesW{\mbox{$\re\!\ll\!W\!\gg$}}
\def\allseriesA{\mbox{$\re\!\ll\!A\!\gg$}}
\def\allseriesA'{\mbox{$\re\!\ll\!A'\!\gg$}}
\def\allseriesZj{\mbox{$\re\!\ll\!Z_j\!\gg$}}
\def\allseriesZbb{\mbox{$\re\!\ll\!Z\cup{\bar{\bar{Z}}}\!\gg$}}
\def\allseriesZZbZbb{\mbox{$\re\!\ll\!Z\cup\bar{Z}\cup{\bar{\bar{Z}}}\!\gg$}}
\def\allseriesrat{\mbox{$\re^{rat}\!\ll\!X\!\gg$}}
%\def\allpolyell{\mbox{$\re^{\ell}\!\!<\!\!X\!\!>$}} % conflicts with above definition
\def\allseriesXxY{\mbox{$\re\!\ll\!X\otimes Y\!\gg$}}
\def\characserie#1{{\bf{#1}^*}} % Symbol for characteristic series


\DeclareMathOperator*{\argmin}{arg\,min}


\newcount\colveccount
\newcommand*\colvec[1]{
	\global\colveccount#1
	\begin{pmatrix}
		\colvecnext
	}
	\def\colvecnext#1{
		#1
		\global\advance\colveccount-1
		\ifnum\colveccount>0
		\\
		\expandafter\colvecnext
		\else
	\end{pmatrix}
	\fi
}

